AVX Timing Side-Channel Attacks against Address Space Layout Randomization

Modern x86 processors support an AVX instruction set to boost performance. However, this extension may cause security issues. We discovered that there are vulnerable properties in implementing masked load/store instructions. Based on this, we present a novel AVX timing side-channel attack that can defeat address space layout randomization. We demonstrate the significance of our attack by showing User and Kernel ASLR breaks on the recent Intel and AMD processors in various environments, including cloud computing systems, an SGX enclave (a fine-grained ASLR break), and major operating systems. We further demonstrate that our attack can be used to infer user behavior, such as Bluetooth events and mouse movements. We highlight that stronger isolation or more fine-grained randomization should be adopted to successfully mitigate our presented attacks.

==> threat.tex <==
\section{Threat model}
\label{sec:threat}

We assume that an attacker can execute arbitrary instructions on the local machine with an unprivileged user account.
The attacker can know the CPU model and the constant offsets of kernel functions.
The process and the kernel are randomly placed by User/Kernel ASLR.
The attacker's goal is to know the addresses of the codes to attempt code reuse attacks.
Even if breaking User/Kernel ASLR can be achieved via memory leak vulnerabilities, we assume that the process or kernel does not have any memory leakages.
For hardware, we assume that the processor supports AVX or AVX2 and is protected by mitigations against the existing side-channel attacks~\cite{intel2018mitigations}.
Since AVX was introduced from the Intel Sandy Bridge (in 2011) and AMD Bulldozer (in 2011) processors, it is reasonable to assume that the vast majority of modern mobile, desktop, server, and cloud systems support AVX or AVX2 by default.

